Pre-supernova O-C shell mergers could produce more $^{44}\mathrm{Ti}$ than the explosion

The formation of $^{44}\mathrm{Ti}$ in massive stars is thought to occur during explosive nucleosynthesis, however recent studies have shown it can be produced during O-C shell mergers prior to core collapse. We investigate how mixing according to 3D macro physics derived from hydrodynamic simulations impacts pre-supernova O-C shell merger nucleosynthesis and if it can dominate explosive supernova production of $^{44}\mathrm{Ti}$ and other radioactive isotopes. We compare a range of observations and models of explosive $^{44}\mathrm{Ti}$ yields to pre-explosive multi-zone mixing-burning nucleosynthesis simulations of an O-C shell merger in a $15~\mathrm{M_\odot}$ $Z=0.02$ stellar model with mixing conditions corresponding to different 3D hydro mixing scenarios. Radioactive species produced in the $\mathrm{O}$ shell have a multi-dex spread in pre-explosive yield predictions across different 3D mixing scenarios of $1.54~\mathrm{dex}$ and $2.14~\mathrm{dex}$ on average depending on mass cut. $^{44}\mathrm{Ti}$ has the largest spread of $4.78~\mathrm{dex}$ and $4.81~\mathrm{dex}$ depending on mass cut. Further, we show that the pre-explosive production of $^{44}\mathrm{Ti}$ can be larger than the explosive production of models and can match observations. Our results also show that 3D mixing physics enhances $^{44}\mathrm{Ti}$ in 1D models without modifying $^{56}\mathrm{Ni}$ yields. We conclude that quantitative predictions of $^{44}\mathrm{Ti}$ and other radioactive species more broadly require an understanding of the 3D hydrodynamic mixing conditions present during the O-C shell merger.

==> vectors.tex <==
%=======================================================================
%
% vectors.tex---some basic vector operators
%
% Requires package bm.sty
%
%=======================================================================

\RequirePackage{bm}
%\RequirePackage{amssymb}
%\RequirePackage{amsbsy}
\newcommand{\bvec}[1]{\ensuremath{\boldsymbol{#1}}} %boldface vector style
\newcommand{\grad}{\bvec{\nabla}} %gradient
\newcommand{\divr}{\nabla \cdot} %divergence
\newcommand{\curl}{\bvec{\nabla \times}} %curl
\newcommand{\lap}{\ensuremath{\nabla^2}} %Laplacian
\newcommand{\btens}[1]{\ensuremath{\boldsymbol{\mathsf{#1}}}}
\newcommand{\vcross}{\bvec{\times}}
\newcommand{\vdot}{\bvec{\cdot}}
\newcommand{\vort}{\ensuremath{|\curl u|}}
\newcommand{\vortsq}{\ensuremath{\vort^2}}
% end vectors.tex

